Quantum Entropy Scoring for Fast Robust Mean Estimation and Improved Outlier Detection

We study two problems in high-dimensional robust statistics: \emph{robust mean estimation} and \emph{outlier detection}. In robust mean estimation the goal is to estimate the mean $\mu$ of a distribution on $\mathbb{R}^d$ given $n$ independent samples, an $\varepsilon$-fraction of which have been corrupted by a malicious adversary. In outlier detection the goal is to assign an \emph{outlier score} to each element of a data set such that elements more likely to be outliers are assigned higher scores. Our algorithms for both problems are based on a new outlier scoring method we call QUE-scoring based on \emph{quantum entropy regularization}. For robust mean estimation, this yields the first algorithm with optimal error rates and nearly-linear running time $\widetilde{O}(nd)$ in all parameters, improving on the previous fastest running time $\widetilde{O}(\min(nd/\varepsilon^6, nd^2))$. For outlier detection, we evaluate the performance of QUE-scoring via extensive experiments on synthetic and real data, and demonstrate that it often performs better than previously proposed algorithms. Code for these experiments is available at https://github.com/twistedcubic/que-outlier-detection .

==> deprecated.tex <==

OLD STUFF HERE

\begin{algorithm}
  \textsc{FastEpoch}$(X_1,\ldots,X_n,w,T,\epsilon,r,\ell)$:\\
  Let $\lambda_0 \leftarrow \textsc{EstimateSpectralNorm}(X_1,\ldots,X_n,w)$.\\
  Let $w^{(0)} \rightarrow w$\\
  For $t = 1,\ldots,T$,
  \begin{enumerate}
    \item Let $\lambda_t \leftarrow \textsc{EstimateSpectralNorm}(X_1,\ldots,X_n,w^{(t-1)})$.
    \item If $\lambda_t \leq \lambda_0/2$, output $w^{(t-1)}$ and terminate.
    \item Otherwise, let $\tau_t,\Phi_{t} \leftarrow \textsc{ComputeScores}(X_1,\ldots,X_n,w^{(1)},\ldots,w^{(t-1)},\Phi_1,\ldots,\Phi_{t-1},\epsilon,r,\ell)$.
    \item Let $w^{(t)} = \textsc{1DFilter}(w^{(t-1)},\tau_t)$\mper
  \end{enumerate}
\vspace{1cm}
\textsc{ComputeScores}$(X_1,\ldots,X_n,w^{(1)},\ldots,w^{(t-1)},\epsilon,r,\ell)$:\\
\begin{enumerate}
  \item For $s \leq t-1$ compute $\mu_s = \tfrac 1 {|w^{(s)}|} \cdot \sum_{i=1}^n w_i^{(s)} X_i$.
  \item Sample a random $\ell \times d$ matrix $\Phi_{t}$ with entries independent from $\cN(0,1/\ell)$.
  \item Compute sketches $\tilde{X_i}^{(s)} = \Phi_{s} (X_i - \mu_s) $ for $s \leq t$.
  \item Let $Y_t = P_{\e/2}^{r} (\sum_{s=1}^t \sum_{i=1}^n w_i^{(s)} (\tilde{X_i}^{(s)})(\tilde{X_i}^{(s)})^\top )^2$.
  \item Compute $\alpha_t = \Tr Y_t$.
  \item Compute $\tau_i = \iprod{X_i - \mu_t , Y_t X_i} / \alpha_t$.
  \item Output $\tau$.
\end{enumerate}
TODO make this right
\end{algorithm}

\begin{fact}[\textsc{EstimateSpectralNorm}]
  For every $d \in N$ and $\e,\delta \in (0,1)$ there is a randomized algorithm which takes a $ d\times d$ symmetric matrix $M$, executes $O(\log d \cdot \log(1/\delta) / \e)$ matrix-vector multiplies and performs $O(d \log (1/\delta))$ additional floating-point operations and with probability at least $1-\delta$ returns $\lambda(M)$ such that $(1-\e) \|M\| \leq \lambda(M) \leq (1+\e) \|M\|$.
\end{fact}
\begin{proof}
  The algorithm is the power method.
  Let $\lambda_1,\ldots,\lambda_n$ be the eigenvalues of $M$.
  Let $g \sim \cN(0,\Id)$.
  Computing $v = (M^t)g$ requires $t$ matrix-vector multiplication operations.
  Notice that $\E \|v\|^2 = \E \iprod{gg^\top, M^{2t}} = \Tr M^{2t} = \sum_{i=1}^n \lambda_i^{2t}$.
  By the Hansen-Wright inequality, $\|v\|^2$ has a sub-exponential tail:
  \[
  \Pr(|\|v\|^2 - \E \|v\|^2| > s) \leq 2 \exp(-c \min(s^2/\|M^{2t}\|_F, s/\|M^{2t}\|))\mper
  \]
  So averaging $n$ independent copies of $v$,
  \[
  \Pr \Paren{ \Abs{\frac 1 n \sum_{i=1}^n \|v_i\|^2 - \E \|v\|^2 } > s} \leq 2 \exp(- c \min(s^2 n / \|M^{2t}\|_F, s n /\|M^{2t}\|))\mper
  \]
  Taking $s = \Tr M^{2t}/2$ and $n = O(\log(1/\delta))$, we find that with probability at least $1-\delta$,
  \[
  \frac 1 2 \Tr M^{2t} \leq \frac 1 n \sum_{i=1}^n \|v_i\|^2 \leq \frac 32 \Tr M^{2t}
  \]
  Noting also that $\lambda_1^{2t} \leq \Tr M^{2t} \leq d \lambda_1^{2t}$, we obtain that with probability $1-\delta$,
  \[
  \frac 12 \lambda_1^{2t} \leq \frac 1 n \sum_{i=1}^n \|v_i\|^2 \leq \frac 32 \cdot d \cdot \lambda_2^{2t}\mper
  \]
  Let $X = (\tfrac 1n \sum_{i=1}^n \|v_i\|^2)^{1/2t}$.
  Then choosing $t = O(\log d / \e)$, we find that $X \in (1 \pm \e) \lambda_1$ with probability at least $1-\delta$.
\end{proof}



\section{Old stuff}

--------------- BELOW THIS LINE BE DEPRECATED ------

\section{Understanding the one dimensional multiplicative weights update}



\section{The maximum entropy certificate}
Let $M = M(w)$ be some PSD matrix, with $\| M \|_2 \geq 10 C$.
For any $U \in \Delta_{n \times n}$ let 
\[
\Ent (U) = - \tr (U \log U) = \sum_{i = 1}^n \lambda_i \log \frac{1}{\lambda_i} 
\]
denote the von Neumann entropy of $U$.
It is well-known that this is a concave operator in $U$.
We wish to find the solution $U$ to the following concave maximization program:
\begin{equation}
\label{eq:max-entropy}
\max_{U \in \Delta_{n \times n}} \Ent (U) ~\mbox{s.t.}~\iprod{U, M} \geq C \; .
\end{equation}

\subsection{In the scalar setting}
Let's pretend that our matrix is diagonal for now i.e. $M = \diag (m_1, \ldots, m_n)$, so that we are in




\section{The Algorithm}
Let $\calX = \{ X_1, \ldots, X_n \} \sim_\eps \normal (\mu, I)$.
WLOG, assume that the true mean $\mu$ satisfies $\| \mu \| \leq O(\eps \sqrt{d})$, and assume that $\| X_i \|_2 \leq O(\sqrt{d \log (n)})$ for all $i \in [n]$.
By trivial methods we may guarantee both of these properties in nearly linear time.
Moreover, let
\[
S_{n, \eps} = \left\{w \in \R^n: \sum_{i = 1}^n w_i = 1 ~\mbox{ and }~ w_i \in \Brac{0, \frac{1}{(1 - \eps) n}} ~\mbox{ for all $i \in [n]$} \right\} \; ,
\]
Notice that for all $w \in S_{n, \eps}$, we have $\| w \|_2 \leq \frac{1}{(1 - \eps) \sqrt{n}}$, that is, $S_{n, \eps} \subset B \Paren{0, \frac{1}{(1 - \eps) \sqrt{n}}}$.

For any symmetric matrix $A$ with singular values $\sigma_1 \geq \sigma_2 \geq \ldots \geq \sigma_d \geq 0$ with corresponding eigenvalues $v_1, \ldots, v_k$, and any $k \geq 1$, let $\| A \|_{\Paren{k}}$ denote the Ky Fan $k$-norm of $A$, namely, the sum of the $k$ largest singular values of $A$, and let $\fS_k (A) = \span \{v_i: \sigma_i \geq \sigma_k \}$ denote the subspace of $\R^d$ spanned by eigenvectors of $A$  with eigenvalue at least the $k$-th largest eigenvalue.

Finally, for any $k \geq 1$, any $\nu \in \R^d$, and any $w \in S_{n, \eps}$, let
\[
\Phi_{k}^\nu (w) = \Phi_{k, \calX}^\nu (w) = \Norm{\sum_{i = 1}^n w_i (X_i - \nu) (X_i - \nu)^\top - I}_{\Paren{k}} \; .
\]
Observe that for any fixed $k, \nu$, the function $w \to \Phi_k^\nu (w)$ is convex in $w$, and moreover, the subdifferential of $\Phi_k^\nu (w)$ at $w$ is given by
\[
\partial_w \Phi_{k}^\nu (w) = \left\{ u \in \R^n : u_i = (X_i - \nu)^\top U (X - \nu)^\top - k \right\} \; ,
\]
where in the RHS of the above expression, $U \in \R^{d \times k}$ is any orthogonal matrix whose columns live in the span of $\fS_k \Paren{\sum_{i = 1}^n w_i (X_i - \nu) (X_i - \nu)^\top}$.
Let $U_k^\nu (w) = U_{k, \calX}^\nu (w)$ denote any such $U$.

Our algorithm will proceed as follows.
Let $V_0^2 = \eps \sqrt{d}$, and let $\nu_0 = 0$.
For $\ell$ starting at $0$ until termination:
\begin{itemize}
\item
Repeatedly run subgradient descent on $\Phi_2^\nu (w)$ until the objective value has decreased by some constant factor.
Let $w^{(\ell + 1)}$ be the resulting $w$.
\item
Set $\nu_{\ell + 1} = \sum_{i = 1}^n w^{(\ell + 1)}_i X_i$, and let $V_{\ell + 1} = V_{\ell} / 2$.
\item
At every iteration of subgradient descent, with $w$ be the current iterate, check if
\[
\sum_{i = 1}^n \Paren{(X_i - \nu)^\top U^\nu_2 (w) (X_i - \nu) - 2}^2 > C R_{\ell - 1} n \log ??? \; ,
\] 
for some universal constant $C > 0$ sufficiently large.
If it is, remove all points $X_i$ with 
\[
\Paren{(X_i - \nu)^\top U^\nu_k (w) (X_i - \nu) - 2}^2 > ???? \; 
\]
from the dataset, and restart the entire process on this truncated data set, i.e. reset $R_{\ell + 1} = \eps \sqrt{d}$ and $\nu_{\ell + 1} = 0$.

\end{itemize}

\section{Concentration Inequalities}

\begin{lemma}
Let $Y_1, \ldots, Y_n \sim \normal (0, I)$.	
\end{lemma}

\section{A general theory of robust estimation?}
Throughout this section, let $D$ be a distribution over $\R^d$ with mean $\mu$ and covariance $I$.
Let $f: \R \to \R_{\geq 0}$ be convex, and for any unit vector $v \in \bS^{d -1}$, define the function $\Psi_v : \R \to \R$ by
\[
\Psi_v = \E_{X \sim D} \Brac{f(\iprod{v, X - \mu}^2)} \; ,
\]
and let $\Psi = \max_{v \in \bS^{d - 1}} \Psi_v (s)$.
The function $f$ and the corresponding functions $\Psi_v, \Psi$ are supposed to capture the ``worst'' tail behavior of the distribution $D$.
Intuitively, the better concentrated $D$ is, the larger we can take $f$ and still have finite $\Psi$.
As a result, the fastest growing $f$ so that this quantity is finite captures the tightest concentration behavior of $D$, and should intuitively characterize the best error we can hope to achieve in a robust setting.

To this end, let
\[
\eta_f (\eps) = \eps \cdot \sqrt{f^{-1} (1 / \eps)} \; .
\]
For instance, when $f(x) = x$, we have $\eta_f (\eps) = \sqrt{\eps}$, and when $f(x) = \exp (x - 1),$ we have $\eta_f (\eps) = \Theta \paren{\eps \sqrt{\log 1 / \eps}}$.
The former is supposed to correspond to the bounded second moment case, and the latter to the Gaussian with known covariance case.
The goal is to naturally interpolate between these two settings: perhaps we can always achieve $\eta_f (\eps)$ using a unified framework.

\subsection{Concentration bounds}

We require analogs of the spectral bounds previously proven in the bounded second moment case.
Specifically, we will prove:
\begin{theorem}
\label{thm:general-conc}
Let $X_1, \ldots, X_n$ be $n$ independent samples from $D$, and let $\eps > 0$ be fixed.
Then, there exists an absolute constant $C$ so that
\[
\Pr \Brac{ \sup_{\| v \|_2 = 1} \frac{1}{n} \sum_{i = 1}^n f \Paren{\iprod{v, X_i - \mu}^2} \one_{f \Paren{\iprod{v, X_i - \mu}^2} < 1 / \eps} > ???} \leq ??? \; .
\]
\end{theorem}
\begin{theorem}
\label{thm:general-conc1}
Let $X_1, \ldots, X_n$ be $n$ independent samples from $D$, and let $\eps > 0$ be fixed.
Suppose that $n = \Omega \Paren{\frac{d}{\eps}}$, and let $a = 1 - O(\eps)$.
Then, we have
\[
\Pr \Brac{ \sup_{\| v \|_2 = 1} \sum_{i = 1}^n \one \Brac{f \Paren{a \iprod{v, X_i - \mu}^2} > 2 / \eps} > 2 \eps n } < ??? \; .
\]
\end{theorem}
\begin{proof}
By Markov's inequality, we have that for any $C > 0$, and for any fixed unit vector $v$, we have $\Pr \Brac{f \Paren{\iprod{v, X_i - \mu}^2} > C \Psi} \leq 1 / C$.
Thus, by a Chernoff bound, we have
\[
\Pr \left[ \sum_{i = 1}^n \one \Brac{f \Paren{\iprod{v, X_i - \mu}^2} > C \Psi} > \frac{2 n}{C} \right] \leq \exp \left( -\frac{C \eps n}{3} \right) \; .
\]
Let $\mathcal{N}$ be an $\eps$-net for the unit sphere of size $(1 / \eps)^{O(d)}$.
By standard arguments it is well-known that such nets exist.
Now, for any fixed $j = 1, 2, \ldots,$, by a union bound, we have
\begin{align*}
\Pr \left[ \sup_{v \in \mathcal{N}_j}\sum_{i = 1}^n \one \Brac{f \Paren{\iprod{v, X_i - \mu}^2} > \frac{1}{ \eps^{j}}} > \frac{C}{\eps_j} \eps n \right] &\leq \Paren{\frac{9}{\eps_j}}^d \exp \left( -\frac{C \eps n / \eps_j}{3} \right) \\
&= \exp \Paren{d \log \frac{9}{\eps_j} - \frac{C \eps n / \eps_j}{3}} \\
&\leq \exp \Paren{- \frac{C \eps n / \eps_j}{6}} \; , 
\end{align*}
for our choice of $n$.
Thus, by a union bound over all $j = 1, 2, \ldots$, we have
\begin{align*}
\Pr \left[\sup_{j, v \in \mathcal{N}_j}\sum_{i = 1}^n \one \Brac{f \Paren{9 \iprod{v, X_i - \mu}^2} > \frac{1}{3 \eps}} > \frac{C}{\eps_j} \eps n \right] &\leq \sum_{j = 1}^\infty \exp \Paren{- \frac{C \eps n / \eps_j}{6}} \\
&\leq 2 \exp \Paren{- \frac{C \eps n}{6}} \; , \numberthis \label{eq:thres-union-bound}
\end{align*}
by our choice of $\eps_j$.

Condition on the event that~\eqref{eq:thres-union-bound} holds.
We claim that in this event, the desired bound follows, which clearly implies the lemma.
For any unit vector $u$, we can always write
\[
u = \sum_{j = 1}^\infty \alpha_j v_j \; ,
\]
where $v_j = v_j (u) \in \mathcal{N}_j$, $\alpha_1 = 1$, and $0 \leq \alpha_j \leq \eps_{j - 1}$.
Let $A = \sum_{j = 1}^\infty \alpha_j$.
Observe that $A \leq (1 + 2\eps_1) \leq 3$.
By Jensen's inequality, we know that 
\begin{align*}
f(\iprod{u, X_i - \mu}^2) &= f \Paren{\Paren{\sum_{j = 1}^\infty \iprod{  \alpha_j v_j, X_i - \mu}}^2} \\
&\leq \sum_{j = 1}^\infty \alpha_j f(A^2 \iprod{v_j, X_i - \mu}^2) \leq \sum_{j = 1}^\infty \eps_{j - 1} f(9 \iprod{v_j, X_i - \mu}^2) \; ,
\end{align*}
where we let $\eps_0 = 1$.
As a result, we know that 
\begin{align*}
\sum_{i = 1}^n \one \Brac{f \Paren{\iprod{v, X_i - \mu}^2} > 1/\eps} \leq \sum_{i = 1}^n \sum_{j = 1}^\infty \one \Brac{f \Paren{9 \iprod{v_j, X_i - \mu}^2} > \frac{1}{3 \eps}} \; .
\end{align*}



% Thus, by a union bound over all $j = 1, 2, \ldots$, we have
% \begin{align*}
% \Pr \left[\sup_{j, v \in \mathcal{N}_j}\sum_{i = 1}^n \one_{f \Paren{\iprod{v, X_i - \mu}^2} < 1 / \eps} > \frac{C}{\eps_j} \eps n \right] &\leq \sum_{j = 1}^\infty \exp \Paren{- \frac{C \eps n / \eps_j}{6}} \\
% &\leq 2 \exp \Paren{- \frac{C \eps n}{6}} \; ,
% \end{align*}
% by our choice of $\eps_j$.

% Now, for any unit vector $u$, we can always write
% \[
% u = \sum_{j = 1}^\infty \alpha_j v_j \; ,
% \]
% $v_j = v_j (u) \in \mathcal{N}_j$, where $\alpha_1 = 1$, and $0 \leq \alpha_j \leq \eps_{j - 1}$.
% Let $A = \sum_{j = 1}^\infty \alpha_j$.
% Observe that $A \leq (1 + 2\eps_1)$.
% THIS IS NOT USEFUL!!!
\end{proof}

For any $S \subseteq [n]$, and any vector $u \in \R^d$, we let $\mu(S) = \frac{1}{|S|} \sum_{i \in S} X_i$, and we let
\[
M(w, u) = \frac{1}{|S|} \sum_{i \in S} \Paren{X_i - u}\Paren{X_i - u}^\top \; .
\]
\noindent
Our algorithm will proceed in epochs.
Given an $\eps$-corrupted dataset $S$,
For epoch $\ell = 1, \ldots, L$, we have a fixed centering vector $\mu^{\Paren{\ell}}$, initially the average of the points in $S$.
Within each epoch, we play matrix multiplicative weights with best response.
That is, for $t = 1, \ldots, T$, given a MMW player action $U_t^{\Paren{s}} \in \Delta_{d \times d}$, we compute the scores
\[
\tau_i = \Iprod{\Paren{X_i - u^{\Paren{s}}} \Paren{X_i - \mu^{\Paren{s}}}, U_t} - 1 \; .
\]
We then find a set of $(1 - \eps) n$ points $S_t^{\Paren{s}}$ with smallest $\abs{\tau_i}$, and we play the response $F_t = M(S_t^{\Paren{s}}, \mu^{(s)})$.
Then, at the end of the epoch, we let $\mu^{\Paren{s + 1}} = \frac{1}{T} \sum_{i = 1}^T \mu(S^{\Paren{s}}_t)$.

